Sample-Near-Optimal Agnostic Boosting with Improved Running Time

Boosting is a powerful method that turns weak learners, which perform only slightly better than random guessing, into strong learners with high accuracy. While boosting is well understood in the classic setting, it is less so in the agnostic case, where no assumptions are made about the data. Indeed, only recently was the sample complexity of agnostic boosting nearly settled arXiv:2503.09384, but the known algorithm achieving this bound has exponential running time. In this work, we propose the first agnostic boosting algorithm with near-optimal sample complexity, running in time polynomial in the sample size when considering the other parameters of the problem fixed.

==> mathstyle.tex <==
\usepackage{bm}

\makeatletter
% \GenerateAlphabetCmds{<prefix>}{<style-command>}
%
% Generates short commands for applying a given style to uppercase letters.
% The commands have the form `\<prefix>A`, `\<prefix>B`, ..., `\<prefix>Z` and are defined as `\<style-command>{A}`, `\<style-command>{B}`, ..., `\<style-command>{Z}`. (Defaults to uppercase letters. One can use `\lowercase` in the style to get lowercase letters.)
% If a command with the same name already exists, it is not redefined. (E.g., if `\calA` is already defined, it is not overwritten.)
%
% Example usage:
% `\GenerateAlphabetCmds{cal}{\mathcal}`
% Defines `\calA`, `\calB`, ..., `\calZ` as short for `\mathcal{A}`, `\mathcal{B}`, ..., `\mathcal{Z}`
\newcommand{\alphacmd@factory}[1]{}
\newcounter{alphacmdcounter}
\newcommand{\GenerateAlphabetCmds}[2]{%
    \renewcommand{\alphacmd@factory}[1]{%
        \expandafter\providecommand\csname #1##1\endcsname{{#2{##1}}}%
    }
    \setcounter{alphacmdcounter}{0}
    \loop
        \stepcounter{alphacmdcounter}
        \edef\alphacmd@ID{\@Alph\c@alphacmdcounter}
        \expandafter\alphacmd@factory\alphacmd@ID
    \ifnum\thealphacmdcounter<26
    \repeat
}

% \GenerateAlphabetCmdsLower{<prefix>}{<style-command>}
%
% Similar to `\GenerateAlphabetCmds`, but generates commands with lowercase letters: `\<prefix>a`, ..., `\<prefix>z` (instead of `\<prefix>A`, ..., `\<prefix>Z`) as short for `\<style-command>{a}`, ..., `\<style-command>{z}` (instead of `\<style-command>{A}`, ..., `\<style-command>{Z}`).
\newcommand{\GenerateAlphabetCmdsLower}[2]{%
    \renewcommand{\alphacmd@factory}[1]{%
        \expandafter\providecommand\csname #1##1\endcsname{{#2{##1}}}%
    }
    \setcounter{alphacmdcounter}{0}
    \loop
        \stepcounter{alphacmdcounter}
        \edef\alphacmd@ID{\@alph\c@alphacmdcounter}
        \expandafter\alphacmd@factory\alphacmd@ID
    \ifnum\thealphacmdcounter<26
    \repeat
}
\makeatother


% General `\mathbb` letters
\GenerateAlphabetCmds{}{\mathbb}

% General `\mathcal` letters
\GenerateAlphabetCmds{c}{\mathcal}

% Random variables
\newcommand*{\StyleRand}{\bm}
\GenerateAlphabetCmds{r}{\StyleRand}
\GenerateAlphabetCmdsLower{r}{\StyleRand}
\newcommand*{\ralpha}{\bm{\alpha}}

% Distributions
\newcommand*{\StyleDist}{\mathcal}
\GenerateAlphabetCmds{d}{\StyleDist}
% Random distributions
\newcommand*{\StyleRandDist}[1]{\bm{\StyleDist{#1}}}
\GenerateAlphabetCmds{rd}{\StyleRandDist}

% Sets
\newcommand*{\StyleSet}{\mathnormal}
\GenerateAlphabetCmds{s}{\StyleSet}
% Random sets
\newcommand*{\StyleRandSet}{\bm}
\GenerateAlphabetCmds{rs}{\StyleRandSet}

% Family of sets
\newcommand*{\StyleFamily}{\mathcal}
\GenerateAlphabetCmds{f}{\StyleFamily}
% Random family of sets
\newcommand*{\StyleRandFamily}[1]{{\bm{\mathcal{#1}}}}
\GenerateAlphabetCmds{rf}{\StyleRandFamily}

% Vectors
\newcommand*{\StyleVec}{\vec}
\GenerateAlphabetCmdsLower{v}{\StyleVec}
\newcommand*{\vzero}{\StyleVec{0}}
\newcommand*{\veps}{{\StyleVec{\eps}}}
% Random vectors
\newcommand*{\StyleRandVec}[1]{\StyleRand{\StyleVec{#1}}}
\GenerateAlphabetCmdsLower{rv}{\StyleRandVec}
\newcommand*{\rvzero}{\StyleRandVec{\vzero}}
\newcommand*{\rveps}{{\StyleRandVec{\veps}}}

% Graphs
\newcommand*{\StyleGraph}{\mathfrak}
\GenerateAlphabetCmds{g}{\StyleGraph}

